MP-RW-LSH: An Efficient Multi-Probe LSH Solution to ANNS in $L_1$ Distance

Approximate Nearest Neighbor Search (ANNS) is a fundamental algorithmic problem, with numerous applications in many areas of computer science. Locality-sensitive hashing (LSH) is one of the most popular solution approaches for ANNS. A common shortcoming of many LSH schemes is that since they probe only a single bucket in a hash table, they need to use a large number of hash tables to achieve a high query accuracy. For ANNS-$L_2$, a multi-probe scheme was proposed to overcome this drawback by strategically probing multiple buckets in a hash table. In this work, we propose MP-RW-LSH, the first and so far only multi-probe LSH solution to ANNS in $L_1$ distance. Another contribution of this work is to explain why a state-of-the-art ANNS-$L_1$ solution called Cauchy projection LSH (CP-LSH) is fundamentally not suitable for multi-probe extension. We show that MP-RW-LSH uses 15 to 53 times fewer hash tables than CP-LSH for achieving similar query accuracies.

==> section/ana_l1-lsh.tex <==
\subsection{Analysis of $L_1$ Multi-Probe LSH}\label{subsec:simu_example_l1}
In this section, we will present simulation results to show that our approximation Eq.~\ref{eq:appro-prob} in Sect.~\ref{subsec:exten-l1} is suitable for multi-probing and using a pre-computed probing sequence, we can significantly accelarate the query process without sacrificing query accuracy.

% To explain the effect of scaling, we will give some simulation results of ``real probing sequences'' and ``pre-computed probing sequences'' to show that scaling does not undermine the quality of multi-probe LSH.  
% Recall that for our hash function (\ref{eq:L1_LSH}), the distance $x_i(\delta)$ to the boundary of slot $h_i(q) + \delta$ would be an uniform random variable from $[0,W]$ and $x_i(-1)+x_i(1) = W$.


Recall that for our hash function Eq.~\ref{eq:L1_LSH}, the distance $x_i(1)$ to the boundary of the $i$-th hash functions is an uniform random variable from $[0,W]$ ($i=1, \ldots, M$) and these distances to boundary are i.i.d., so we simulate these $M$ values $x_1(1),\ldots, x_M(1)$ and calculate the distance to the opposite boundary based on the equality $x_i(1)+x_i(-1)=W$.
We calculate the success probability of the top-T hash buckets with different $L_1$ distance value $d$.
We refer to the summation of these success probabilities as $\mathcal{P}(d)$, which is actually the probability of finding the point $p$ in one hash table after probing extra T hash buckets given a query point $q$ and their $L_1$ distance equal to $d$.
Larger probability $\mathcal{P}(d)$ directly results in a higher query accuracy. 

Table~\ref{tab:rw_gauss_probability} reports $\mathcal{P}(d)$ from 1000 simulations in real sequence and pre-computed sequence of our ToW-based LSH and the converged Gaussian LSH, respectively.
The number of hash functions $M$ is set to a typical value 10 and the bucket width $W$ is set to 8, which can achieve near optimal LSH quality $\rho$ for $r_1=6$ and $r_2 =12$ for ToW-based LSH. 

Apprantly Table~\ref{tab:rw_gauss_probability} shows that the summation of success probabilities of our ToW-based LSH is very close to the converged Gaussian LSH in ``pre-computed sequence'', with less than $10\%$ relatively difference.
This suggests that our approximation in Eq.~\ref{eq:appro-prob} will only have trivial effect on the query accuracy.
Also, the table shows that in ToW-based LSH, the use of pre-computed probing sequence will result in a tiny reduction on the query accuracy - the relative difference of $\mathcal{P}(d)$ between real probing sequence and precomuted sequence is less than $10\%$.
We draw a histogram for the success probability of Top-$40$ buckets as shown in Fig.~\ref{fig:succ_prob_rw_40} to explain the details of difference between pre-computed seqence and real sequence when $d=6$ and set $T=30$.
With the use of pre-computed sequences, approximately 3-4 perturbation vectors in real probing sequence are missing.
However, the histrogram shows that these missing vectors are usually not top-$10$ buckets, which are the main part of $\mathcal{P}(d)$.
Therefore, missing 3-4 perturbation vectors in real sequence will not significantly undermine the total success probability $\mathcal{P}(d)$.

Although query accuracy of real sequence is slightly better than pre-computed sequence, calculating query-wise probing sequence is time-consuming.
The computation of pre-determined probe sequence only needs sorting the perturbation vectors based on their distance, and so the time required for the computation can be small.
From our 1000 simulation results, the time to generate real sequence is approximately 906 times greater than the time to produce pre-computed sequence. For Gaussian LSH, the time to generate real sequence is approximately 71 times greater than the time to produce sequence from sorted squared distances.
\textbf{HUAYI: A sentence probably here or somewhere to explain query time: Query time contains three parts, first part is to calculate hash values and generate the distance to each boundary(not measure here), second is to find the probing hash buckets(time measure here), third is to probe the points from hash buckets. The second part is almost the same order as first part if pre-computed, the time third-part depends on the datasets and is larger than the first and second parts. The second part time if precompute can be negligible in large dataset. However, time to computing the real sequence is still larger than probing points even for 1 million large dataset.} 

% Table \ref{tab:rw_gauss_real} shows the real summation probability of random walk and the converging Gaussian distribution $\mathcal{N}(0,d)$ in real probing sequences.
% The absolute difference is smaller for larger probability values.
% For example, when $d \geq 16$, the absolute difference is smaller than $7\%$.
% More importantly, we see that the ratio of the random-walk based probability to the Gaussian distribution is roughly between 1.1 and 1.2 for each combination of $d$ and $T$.
% The phenomenon can be attributed to the fact that Gaussian distributions have fat tails, which are unreachable using random walks.
% That is, the range of a random walk is $[-d,d]$ while the range of a Gaussian is $[-\infty,\infty]$.
% The truncation of tails and the relative similarity are advantageous to us because our goal is to establish an approximation of the local neighborhood of a given query, not an approximation of the entire Gaussian population.
% The truncation necessary distorts the distribution, but the use of multiple hash functions will help us avoid following false positives.
 
%% Table \ref{tab:rw_gauss_real} shows the real summation probability of random walk and the converging Gaussian distribution $\mathcal{N}(0,d)$ in real probing sequences.
%% From the table, we see that the ratio of the random-walk based probability to the Gaussian distribution is roughly between 1.1 and 1.2 for each combination of $d$ and $T$.
%% The absolute difference is smaller for larger probability values.
%% For example, when $d \geq 16$, the absolute difference is smaller than $7\%$.
%% The phenomenon can be attributed to the fact that Gaussian distributions have fat tails, which are unreachable using random walks.
%% That is, the range of a random walk is $[-d,d]$ while the range of a Gaussian is $[-\infty,\infty]$.
%% , the random walk variable can not reach as far as a Gaussian random variable, therefore for random walk points would fall in the hash bucket $g(p)=g(q)+\Delta$, with just several +1 or -1 in hash perturbation vector $\Delta$. Because of this, our LSH scheme based on random walk is still suitable for multi-probe framework, even it is no close to Gaussian in small distance.
\begin{table}[htb]
\centering
 \caption{$\mathcal{P}(d)$ from 1000 simulations, $M=10$, $W=8$
 } \label{tab:rw_gauss_probability}
 \begin{tabular}{@{}l|r r r|r r r@{}}
\hline
  \multicolumn{7}{c}{ToW-based LSH} \\
 \hline
 & \multicolumn{3}{c|}{Real Sequence} & \multicolumn{3}{c}{Pre-Computed}\\
  \hline
 Distance & T=30 & T=60 & T=100 & T=30 & T=60 & T=100 \\ 
 \hline
6   & 0.50  & 0.63 & 0.72 & 0.46  & 0.58 & 0.67 \\
8   & 0.36 & 0.48 & 0.57 & 0.33 & 0.43 & 0.52 \\
12   & 0.19 & 0.27 & 0.34 & 0.17  & 0.24 & 0.31 \\ 
16   & 0.10  & 0.15 & 0.20 & 0.09  & 0.14 & 0.19 \\ 
  \hline
  \multicolumn{7}{c}{Gaussian} \\
 \hline
 \multicolumn{4}{r}{Real Sequence} & \multicolumn{3}{c}{Pre-Computed}\\
  \hline
 Distance & T=30 & T=60 & T=100 & T=30 & T=60 & T=100 \\ 
 \hline
6   & 0.48  & 0.61 & 0.70 & 0.46  & 0.58 & 0.67 \\
8   & 0.35 & 0.46 & 0.55 & 0.33 & 0.44 & 0.53 \\
12   & 0.18 & 0.26 & 0.33 & 0.17  & 0.25 & 0.31 \\ 
16   & 0.10  & 0.15 & 0.20 & 0.10  & 0.14 & 0.19 \\ 
  \hline
 \end{tabular}
\end{table}

\begin{figure}
\centering
\begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=1.1\textwidth]{figures/hist_rw_v2}
    \caption{ToW-based LSH}\label{fig:succ_prob_rw_40}
\end{subfigure}%
\begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=1.1\textwidth]{figures/hist_cauchy_v2}
    \caption{Cauchy-based LSH} \label{fig:succ_prob_cauchy_40}
\end{subfigure}
\caption{Success probabilities of Top-40 buckets when $d$=6}\label{fig:succ_prob_40}
\end{figure}


% In table \ref{tab:rw_gauss_pre}, we report the summation probability of random walk and Gaussian in the pre-computed probing sequence. In contrast with table \ref{tab:rw_gauss_real}, the pre-computed sequence can achieve almost the same accuracy (less than $1\%$ difference) as real probing sequence in Gaussian distribution. For random walk, the difference of $\mathcal{P}(d)$ is less than $2\%$ between pre-computed probing sequence and real probing sequence, which is relatively small in terms of the summation of probabilities $\mathcal{P}(d)$. Furthermore, as explained before, our random walk scheme could achieve slightly better accuracy than Gaussian scheme, because of this advantage, using the pre-computed probing sequence based on Gaussian would not undermine the accuracy of random walk. 
% The 40-th buckets over first bucket success probability ratio for random walk is $0.0544$, for cauchy is $0.1250$.


% From this table, we can see that the ``scaling trick'' could increase the multi-probe quality. 


==> section/needed.tex <==
% Table~\ref{tab:cauchy_probability} clearly shows, for the same $T$ and $d_1$, the $\mathcal{P_T}(d_1)$
% is approximately one order of magnitude smaller than that under template-generated multi-probe RW-LSH. For example, when $d = 6$, the ... value under ... is only ..., ..., ... for T = ..., ..., ..., respectively;  in comparison, the ... values under ??? 
% are ..., ..., and ... respectively, which are one order of magnitude larger. 

{\color{red} Huayi Paragraph to explain query time of our RW-MPLSH is not as good as cauchy: Here, we give a example to show the quality difference between our LSH scheme and Cauchy based LSH scheme. For example, 
when $r_1=6, r_2=12$,  for our $L_1$-LSH, given $W=8$,we have $p_0(r_1)=0.7656$, $p_0(r_2)=0.6633$ and $\rho=0.6506$. In contrast, for Cauchy-based LSH, given $W=20$, we have $p_0(r_1)=0.5763$, $p_0(r_2)=0.4021$, and $\rho=0.6050$ from Eq.~\ref{eq:coll_prob_l_1}. In terms of LSH quality, our RW-based LSH has slightly larger quality than Cauchy-based LSH. Therefore, in basic LSH framework, our RW-based LSH will have worse performance than Cauchy based LSH since the number of hash tables is $O(n^{\rho})$ and the tradeoff between query accuracy and query time is $O(n^{\rho})$ as described in Sect.~\ref{subsec:lsh_background}. However, in the multi-probe framework, we have successfully reduced the number of hash tables from $O(n^{\rho})$ to a constant. So the quality of LSH will not affect space complexity anymore. As for the tradeoff between query accuracy and query efficiency of RW-MPLSH, it is also related with the LSH quality $\rho$. For the epicenter bucket, in order to find the true nearest neighbor with probability $p_0(r_1)^M$ (query accuracy), we need to probe extra $O(p_0(r_2)^Mn)$ (query time) points in this bucket. For the $T$-th likely bucket, in order to find the true nearest neighbor (with probability $p_T(r_1)^{M}$), we need to probe extra $O(p_T(r_2)^Mn)$ points in this bucket. Since the $\frac{log(1/p_0(r_1))}{log(1/p_0(r_2))}$ is similar to $\frac{log(1/p_T(r_1))}{log(1/p_T(r_2))}$. So the tradeoff of query time and query accuracy of RW-MPLSH is also related with its LSH quality $\rho$, since our quality is close to the Cauchy-based LSH, the query time of our RW-LSH with multi-probe will be slightly larger than Cauchy-based LSH when achieving similar query accuracy, this is corresponding with our evaluation results in Sect.~\ref{sec:eva}}.

==> section/scheme.tex <==
\section{$L_1$-LSH HASHING}\label{sec:lsh-scheme}
% {\bf Mitsu: perhaps we need to say what ToW is and what EEC is...}
% {\bf Mitsu: perhaps we need to say we are defining our $L_1$-locality sensitive hashing ($L_1$-LSH).}
In this section we describe our extension of a ToW-based LSH family for Hamming distance described in\cite{gong2020idec} to an LSH family for $L_1$ distance. All description is focusing on one hash table.

% {\bf Mitsu: Let us recall the definition of the $L_1$ (Manhattan) distance.
% In this section, we will let $U$ denote our universe of vectors - a set of $d$-dimensional vectors.}

A one-dimensional random walk is the random discrete-time process where an object moves along a one-dimension grid starting from the origin $0$ and at each step, it chooses to either increase its position by $1$ or decrease its position by $1$ with probability $1/2$.
A one-dimensional random walk can be represented as an infinite sequence, each of whose elements is either $-1$ or $+1$ chosen independently and uniformly at random.
% For all positive integer $t$, a $t$-step one-dimensional random-walk can be represented as a $t$-tuple whose elements are from $\{ -1, +1 \}$, where for each $i, 1\leq i\leq t$, the $i$-th entry of the tuple represents the change in the position at step $i$.
% Let $\mathcal{R}_t$ denote the set of all $t$-step one-dimensional random walks, and let $\mathcal{R}$ denote the $\cup_{t \geq 1} \mathcal{R}_t$.
% For each $t\geq 1$, we assume a uniform distribution over the elements of $\mathcal{R}_t$, that is, the entries of the tuples are chosen independently and uniformly at random from $\{ -1, + 1 \}$.
% For all $t, t'$ such that $1\leq t' < t$, the distribution of the random walks constructed from $\mathcal{R}_t$ by taking the first $t'$ entries is equivalent to the distribution of the random walks $\mathcal{R}_{t'}$.
% For all $t$, $\ell$, $0\leq \ell\leq  t$, and all $t$-step random walks $r = (r_1, \ldots, r_t)$, $r(\ell)$ denotes the position of the object with the walk $r$ after $\ell$ steps; that is, $r(\ell) = r_1 + \cdots + r_\ell$.
Let $\tau = (\tau^{(1)}, \tau^{(2)}, \ldots )$ be a one-dimensional random walk and let $t \geq 0$.
By $\tau(t)$, we denote the position after $t$ steps in the random walk $\tau$; that is, $\tau(t) = \tau^{(1)} + \cdots + \tau^{(t)}$.


Let $x = (x_1, x_2, \ldots, x_n)$ be an $n$-dimensional vector whose elements are all nonnegative integers.
Let $R = (\tau_1, \ldots, \tau_n)$ be a tuple of $n$ independent random walks.
We define $R(x) = \sum_{i=1}^n \tau_i(x_i)$.
As in Eq.~\ref{eq:lsh-l_p}, we add an offset $b$ to the value and then scale it by dividing it by $W$,
\begin{equation}
\phi_{R,b}(x) = \left\lfloor \frac{R(x) + b}{W} \right\rfloor
\label{eq:L1_LSH}
\end{equation}
where $W$ is a positive integer called the bucket width \cite{Huang_QALSH_2015} and $b$ is a nonnegative real number uniformly drawn from $[0,W]$ called the offset \cite{Datar_LocalitysensitiveHashing_2004}.
This $\phi_{R,b}$ is the format of the hash functions we will use in this paper.
The quantity $W$ is a predetermined constant.
In our scheme, we use multiple groups of hash functions.
The parameters we found the hash functions are chosen independently.
In other words, to deploy some $M$ hash functions $h_1, \ldots, h_M$, we choose $n\cdot M$ independent random walks, dividing them into $M$ tuples of size $n$, $R_1, \ldots, R_M$, choose $M$ independent offsets $b_1, \ldots, b_M$, and define for each $i$, $h_i = \phi_{R_i,b_i}$; and if we need to use multiple groups of such $M$ hash functions, the selections are made independently of other groups.

\textbf{Huayi: Not sure where to put this paragraph. I am not sure how to express $R(\alpha) - R(\beta)$ here, the difference between summation of $2nM$ independent random walks.} In our implementation, we precompute these $nM$ independent random walks for query efficiency. Computing the summation of $t$ steps random walk is known as ``range-sum'' problem, Feigenbaum \textit{et al.}~\cite{Feigenbaum_ApproximateL1Difference_2003} propose an sketching algorithm for estimating $t$ steps random walk.  However, this sketching algorithm only estimate the squared value of $t$ steps random walk \textbf{Huayi: I think 4-wise independent is hard to understand here. We can just say it approximate $z^2$ as described in Feigenbaum's paper.} rather than the first-moment value as required in our scheme. We have tested this sketch and find it is not a LSH. Efficiently computing $t$ steps random walk required by our LSH is still a open problem. 


\begin{comment}
It can be shown, using the results in~\cite{Datar_LocalitysensitiveHashing_2004}, that this 
LSH family is $(r_1, r_2, p(r_1), p(r_2))$-sensitive, where the collision probability function $p(\dot)$ is
\begin{equation}\label{eq:collision-prob-trad}
  p(s) = \sum_{t=0}^w(1-\frac{t}{w})\mathbf{Pr}[|Y_s|= t],
\end{equation}
%%% http://www2.math.uu.se/~sea/kurser/stokprocmn1/slumpvandring_eng.pdf
where 
\begin{equation*}\label{eq:rw-prob}
\mathbf{Pr}[|Y_s|= t]=\begin{cases}\binom{s}{s/2}\big{(}\frac{1}{2}\big{)}^s&\mbox{ if } t = 0\\\binom{s}{(s+t)/2}\big{(}\frac{1}{2}\big{)}^s + \binom{s}{(s-t)/2}\big{(}\frac{1}{2}\big{)}^s&\mbox{ otherwise}\end{cases}.
\end{equation*}
Here we define $\binom{n}{x} = 0$ when $x$ is not an integer.
For example, given $w=4$, 
when $r_1=5, r_2=10$, we have $p_1=0.5469$, $p_2=0.4189$, and $\rho=0.6937$.

Here $p(r)$ 
is the probability for two points $\alpha$ and $\beta$ that are $r$ apart in Hamming distance
(i.e., $r=\|\alpha,\beta\|_H$) to be hashed to the same value.  
\end{comment}

% {\bf MITSU: $W$ versus $w$, which do we want to use?}

% Now we calculate the quality of the LSH family we have just defined by deriving its collision probability; i.e., the probability of two points $\alpha,\beta$ have identical hash values (assuming that $R$ and $b$ are chosen uniformly at random).
%when the hash function is uniformly randomly
%drawn from this family. 
%   For  
% a ToW sum $\Psi(\cdot)$ with 
% random $\pm 1$ vector $\psi$, $\Psi(\alpha)-\Psi(\beta)=\langle \alpha - \beta, \psi\rangle$ 
% a $\psi(\cdot)$ with the same random-walk family $R$, $\psi(\alpha)-\psi(\beta)$ 
%
% has the same distribution as the ``distance''
% from the starting point in an $d$-step simple random walk. More precisely, it is distributed as $Y_d=\sum_{i=1}^d X_i$ where
% Now we calculate the collision probability.
Let $\alpha$ and $\beta$ be two $n$-dimensional vectors whose elements are nonnegative integers.
Let $d=\|\alpha,\beta\|_1$. 
Since $\alpha$ and $\beta$ take upon coordinate-wise independent common random walks.
$R(\alpha) - R(\beta)$ follows the same distribution as the result of a single $d$-step one-dimensional random walk.
% Huayi: This part could be comment out if needed
Because our hash function uses an offset $b$ and a bucketing with width $W$, $\phi_{R,b}(\alpha) = \phi_{R,b}(\beta)$ if and only if
\begin{itemize}
\item[(i)]
the absolute difference $\ell$ between $R(\alpha)$ and $R(\beta)$ must satisfy $0 \leq \ell \leq  W$, and
\item[(ii)]
the offset $b$ must move the two values in the same bucket.
\end{itemize}
Given that (i) holds, the number of possible values for $b$ to achieve (ii) is $W - \ell$.
% Comment out end here.
Following the results in~\cite{Datar_LocalitysensitiveHashing_2004}, we obtain the collision probability $p(d)$ as
\begin{equation}\label{eq:coll_prob}
\sum_{\ell=0}^{W}\left(1-\frac{\ell}{W}\right)\mathbf{Pr}[|Y_d| = \ell]
\end{equation}
where
\begin{equation*}\label{eq:rw-prob}
\mathbf{Pr}[|Y_d| = \ell]=\begin{cases}
	\binom{d}{d/2}\big{(}\frac{1}{2}\big{)}^d
	& \mbox{ if } \ell = 0 \\
	\binom{d}{(d+\ell)/2}\big{(}\frac{1}{2}\big{)}^d + \binom{d}{(d-\ell)/2}\big{(}\frac{1}{2}\big{)}^d
	& \mbox{ if } \ell\leq d\\
	0
	& \mbox{ otherwise}\end{cases}
\end{equation*}
Here we define $\binom{n}{x} = 0$ when $x$ is not an integer.

As shown in Appendix~\ref{sec:appendix}, when $W$ is an even integer, the collision probability $p(d)$ decreases
monotonically with all the even integer distance $d=\|\alpha,\beta\|_1$. \textbf{HUAYI no LSH conditions: When $W$ is an odd integer, the collision probability is not monotonically decreasing.
For an odd distance $r_1$, there exists special cases that $p_1=p_2$ (when $r_2=r_1+1$).}Thus, this hash family can be viewed as a special $(r_1, r_2, p_1, p_2)$-sensitive
LSH, where $p_1=p(r_1), p_2=p(r_2)$ and $r_1, r_2$ are both even integers. 


\begin{comment}
In contrast, the standard LSH solution for $L_1$ in \cite{Datar_LocalitysensitiveHashing_2004} based on Cauchy random projection has the collision probability $p(d)$ for $L_1$ distance $d$ as follows:
 \begin{equation}
p(d) = \frac{2}{\pi}\arctan\left(\frac{W}{d}\right)
 - \frac{d}{\pi W}\ln\left(1+\left(\frac{W}{d}\right)^2\right)
\label{eq:succ_prob_cauchy}
\end{equation}
where $W$ is the bucket width defined in Section \ref{subsec:lsh_background}. 
\end{comment}


\textbf{HUAYI: We might need to change the value of $W$ to be different here.}Here, we give a example to show the quality difference between our LSH scheme and Cauchy based LSH scheme. For example, given $w=16$, 
when $r_1=6, r_2=12$,  for our $L_1$-LSH, we have $p_1=0.8828$, $p_2=0.8308$, and $\rho=0.6725$. In contrast, from Eq.~\ref{eq:coll_prob_l_1}, we have $p_1=0.5217$, $p_2=0.3464$, and $\rho=0.6137$. Therefore, in basic LSH framework, our LSH will have worse performance than Cauchy based LSH. However, our LSH has much larger collision probability $p_1$ than standard LSH for $L_1$. And this value is more important than quality in multi-probe framework, as we will show in Sect. \ref{subsec:simu_example_l1}.

We note that the scheme we have presented could apply only to nonnegative even integer vectors.
The limitation can be overcame with some simple adjustments.
%%%% we can do some transformations of datasets to make our applicable on real world datasets without changing ANN-$L_1$ results.
Recall the definition of $L_1$ distance (Definition~\ref{def:l_p}).
For any two $n$-dimensional vectors $\bf{x}$ and $\bf{y}$, any real number $c$, and for any $n$-dimensional vector $\bf{a}$ having the same constant $a$ in each dimension, we have $\|c\mathbf{x},c\mathbf{y}\|_1 = c*\|\mathbf{x},\mathbf{y}\|_1$ and $\|\mathbf{x}+\mathbf{a},\mathbf{y}+\mathbf{a}\|_1 = \|\mathbf{x},\mathbf{y}\|_1$.
Based on these properties, we can adjust the scheme as follows:
First, if the data may contain a negative value, we add a large constant to each coordinate of each vector to ensure that all entries are positive.
The value we add can be the absolute value of the minimum value in the dataset.
Second, if the entries of the dataset are not integral, we can multiply the whole data set with some positive integer (such as $1000$) to scale up and approximate them to integer values.
Third, we multiply the entire set by $2$ to ensure that every entry is an even number.
Note that the first step preserves the ordering generated by the $L_1$ distance values.
The second step may generate tiny differences in the order due to rounding.
The third one preserves the ordering.
We call this transformation of dataset as ``scaling trick'' and we will discuss them in details in Section ? (experiment section).   

% This property suggests that we can multiply 
% the whole database with a scaling number $a$ (typically $a=2$) without changing the order of $L_1$ distance in the database. We call this as ``scaling trick'' and we would use scaling to avoid the special cases of $L_1$-LSH in Section \ref{sec:lsh-scheme}; simultaneously, this will also make the approximation (\ref{eq:appro-prob}) in Section \ref{subsec:exten-l1} more accurate. 




% Note that this $\rho$ is larger ({\it i.e.}, lower in quality) than the lower bound ({\it i.e.}, best possible) quality value of roughly $1/2$ ($=r_1/r_2$).  However, as we will soon show, we can use the multi-probe method to further improve this quality to much better average query time complexity and index space complexity, which is better than traditional Cauchy method.


